The present-day mass function of the Quintuplet cluster

Context: The stellar mass function is a probe for a potential dependence of star formation on the environment. Only a few young clusters are known to reside within the Central Molecular Zone and can serve as testbeds for star formation under the extreme conditions in this region. Aims: We determine the present-day mass function of the Quintuplet cluster, a young massive cluster in the vicinity of the Galactic centre. Methods: We use two epochs of high resolution near infrared imaging data obtained with NAOS/CONICA at the ESO VLT to measure the individual proper motions of stars in the Quintuplet cluster in the cluster reference frame. An unbiased sample of cluster members within a radius of 0.5 pc from the cluster centre was established based on their common motion with respect to the field and a subsequent colour-cut. Initial stellar masses were inferred from four isochrones covering ages from 3 to 5 Myr and two sets of stellar evolution models. For each isochrone the present-day mass function of stars was determined for the full sample of main sequence cluster members using an equal number binning scheme. Results: We find the slope of the present-day mass function in the central part of the Quintuplet cluster to be alpha = -1.66+-0.14 for an approximate mass range from 5 to 40M_Sun, which is significantly flatter than the Salpeter slope of alpha = -2.35. The flattening of the present-day mass function may be caused by rapid dynamical evolution of the cluster in the strong Galactic centre tidal field. The derived mass function slope is compared to the values found in other young massive clusters in the Galaxy.

==> cp-aa.tex <==
% This is cp-aa.ini, the INITEX file to create a format file for
% the Springer journal Astronomy & Astrophysics, based on plain TeX,
% using Computer Modern fonts                           version 3.0
%                                (earlier versions were called aa.cmm)
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\catcode`\{=1 % left brace is begin-group character
\catcode`\}=2 % right brace is end-group character
\catcode`\#=6 % hash mark is macro parameter character
%%% removed from cp-aa.ini:
%\let\x=\input \def\input#1 {\let\input=\x \let\x=\undefined}
%
\let\qayb=\font
\def\font#1=#2 {\def\qayba{#1}\def\qaybb{#2}
                \def\qaybf{\preloaded}
                \def\qaybg{\tenrm}\def\qaybh{\tenex}
                \def\qaybu{cmr7}\def\qaybv{cmtt10}\def\qaybw{cmssbx10}
                \ifx\qayba\qaybg \qayb#1=#2
                \else\ifx\qayba\qaybh \qayb#1=#2
                \else\ifx\qayba\qaybf
                  \ifx\qaybb\qaybu \qayb#1=#2
                  \else\ifx\qaybb\qaybv \qayb#1=#2
                  \else\ifx\qaybb\qaybw \qayb#1=#2 \fi\fi\fi
                \fi\fi\fi}
%
\let\qayc=\skewchar \def\skewchar#1=#2 {\relax}
\let\qayd=\textfont \def\textfont#1=#2{\relax}
\let\qaye=\scriptfont \def\scriptfont#1=#2{\relax}
\let\qayf=\scriptscriptfont \def\scriptscriptfont#1=#2{\relax}
%
%\x plain                                        %%% removed from cp-aa.ini
%
\let\font=\qayb \let\qayb=\undefined
\let\skewchar=\qayc  \let\qayc=\undefined
\let\textfont=\qayd  \let\qayd=\undefined
\let\scriptfont=\qaye  \let\qaye=\undefined
\let\scriptscriptfont=\qayf  \let\qayf=\undefined
%
\def\fonttype{cm}              
%\input hyphen                                   %%% removed from cp-aa.ini
\def\Initexing{}               
\font\sevenrm=cmr7
\font\fiverm=cmr5
\font\teni=cmmi10 % math italic
\font\seveni=cmmi7
\font\fivei=cmmi5
\font\tensy=cmsy10 % math symbols
\font\sevensy=cmsy7
\font\fivesy=cmsy5
\font\tenbf=cmbx10 % boldface extended
\font\sevenbf=cmbx7
\font\fivebf=cmbx5
\font\tentt=cmtt10 % typewriter
\font\tenit=cmti10 % text italic

\skewchar\teni='177 \skewchar\seveni='177 \skewchar\fivei='177
\skewchar\tensy='60 \skewchar\sevensy='60 \skewchar\fivesy='60

\textfont0=\tenrm \scriptfont0=\sevenrm \scriptscriptfont0=\fiverm
\textfont1=\teni \scriptfont1=\seveni \scriptscriptfont1=\fivei
\textfont2=\tensy \scriptfont2=\sevensy \scriptscriptfont2=\fivesy
\textfont3=\tenex \scriptfont3=\tenex \scriptscriptfont3=\tenex
\textfont\itfam=\tenit
\textfont\bffam=\tenbf \scriptfont\bffam=\sevenbf
\scriptscriptfont\bffam=\fivebf
\textfont\ttfam=\tentt
\rm
% This is values.aa
% i.e. Values of package AA
% it contains sizes and measures specific for this macro package
% indention of equations
\newskip\mathindent      \mathindent=0pt
% \titlea
\newskip\tabefore \tabefore=20pt plus 10pt minus 5pt      % space above
\newskip\taafter  \taafter=10pt                           % space below
\newskip\tabaselineskip
\tabaselineskip=20pt
% \titleb
\newskip\tbbeforeback    \tbbeforeback=-20pt              % corrective space to a \titlea
\newskip\tbbefore        \tbbefore=17pt plus 7pt minus3pt % spaceabove
\newskip\tbafter         \tbafter=8pt                     % space below
\newskip\tbbaselineskip
\tbbaselineskip=17pt
% \titlec
\newskip\tcbeforeback    \tcbeforeback=-3pt               % corrective space to a \titleb
\advance\tcbeforeback by -10pt                            % corrective space to a \titleb
\newskip\tcbefore        \tcbefore=10pt plus 5pt minus 1pt% space above
\newskip\tcafter         \tcafter=6pt                     % space below
% \titled
\newskip\tdbeforeback    \tdbeforeback=-3pt                  % corrective space to a \titlec
\advance\tdbeforeback by -10pt                               % corrective space to a \titlec
\newskip\tdbefore        \tdbefore=10pt plus 4pt minus 1pt   % space above
% \petit
\newskip\petitsurround
\petitsurround=6pt\relax
% \ack
\newskip\ackbefore      \ackbefore=10pt plus 5pt             % space above
\newskip\ackafter       \ackafter=6pt                        % space below
% indention of lists
\newdimen\itemindent    \newdimen\itemitemindent
\itemindent=1.5em       \itemitemindent=2\itemindent
% This is cmlayout.tex
% it sets up some measures and defines macros needed by the font
% selection
\catcode`@=11    % use @ as a normal character
\normallineskip=1pt
\normallineskiplimit=0pt
\newskip\ttglue%
\def\ifundefin@d#1#2{%
\expandafter\ifx\csname#1#2\endcsname\relax}
%
\def\getf@nt#1#2#3#4{%
\ifundefin@d{#1}{#2}%
\global\expandafter\font\csname#1#2\endcsname=#3#4%
\fi\relax
}
\newfam\sffam
\newfam\scfam
\def\makesize#1#2#3#4#5#6#7{%
%%% these fonts cannot be loaded dynamically, because there
%%% is no macro we can overload
 \getf@nt{rm}{#1}{cmr}{#2}%
 \getf@nt{rm}{#3}{cmr}{#4}%
 \getf@nt{rm}{#5}{cmr}{#6}%
 \getf@nt{mi}{#1}{cmmi}{#2}%
 \getf@nt{mi}{#3}{cmmi}{#4}%
 \getf@nt{mi}{#5}{cmmi}{#6}%
 \getf@nt{sy}{#1}{cmsy}{#2}%
 \getf@nt{sy}{#3}{cmsy}{#4}%
 \getf@nt{sy}{#5}{cmsy}{#6}%

%%% skewchar
 \skewchar\csname mi#1\endcsname ='177
 \skewchar\csname mi#3\endcsname ='177
 \skewchar\csname mi#5\endcsname ='177
 \skewchar\csname sy#1\endcsname ='60
 \skewchar\csname sy#3\endcsname ='60
 \skewchar\csname sy#5\endcsname ='60

\expandafter\def\csname#1size\endcsname{%
 \normalbaselineskip=#7
 \normalbaselines
 \setbox\strutbox=\hbox{\vrule height0.75\normalbaselineskip%
    depth0.25\normalbaselineskip width0pt}%
 %
%%% "roman"
 \textfont0=\csname rm#1\endcsname
 \scriptfont0=\csname rm#3\endcsname
 \scriptscriptfont0=\csname rm#5\endcsname
    \def\oldstyle{\fam1\csname mi#1\endcsname}%
%%% "mathit"
 \textfont1=\csname mi#1\endcsname
 \scriptfont1=\csname mi#3\endcsname
 \scriptscriptfont1=\csname mi#5\endcsname
%%% "mathsy"
 \textfont2=\csname sy#1\endcsname
 \scriptfont2=\csname sy#3\endcsname
 \scriptscriptfont2=\csname sy#5\endcsname
%%% "mathex"
 \textfont3=\tenex\scriptfont3=\tenex\scriptscriptfont3=\tenex
   \def\rm{%
 \fam0\csname rm#1\endcsname%
   }%
   \def\it{%
 \getf@nt{it}{#1}{cmti}{#2}%
 \textfont\itfam=\csname it#1\endcsname
 \fam\itfam\csname it#1\endcsname
   }%
   \def\sl{%
 \getf@nt{sl}{#1}{cmsl}{#2}%
 \textfont\slfam=\csname sl#1\endcsname
 \fam\slfam\csname sl#1\endcsname}%
   \def\bf{%
 \getf@nt{bf}{#1}{cmbx}{#2}%
 \getf@nt{bf}{#3}{cmbx}{#4}%
 \getf@nt{bf}{#5}{cmbx}{#6}%
 \textfont\bffam=\csname bf#1\endcsname
 \scriptfont\bffam=\csname bf#3\endcsname
 \scriptscriptfont\bffam=\csname bf#5\endcsname
 \fam\bffam\csname bf#1\endcsname}%
   \def\tt{%
 \getf@nt{tt}{#1}{cmtt}{#2}%
 \textfont\ttfam=\csname tt#1\endcsname
 \fam\ttfam\csname tt#1\endcsname
 \ttglue=.5em plus.25em minus.15em
   }%
  \def\sf{%
\getf@nt{sf}{#1}{cmss}{10 at #2pt}%
\textfont\sffam=\csname sf#1\endcsname
\fam\sffam\csname sf#1\endcsname}%
   \def\sc{%
 \getf@nt{sc}{#1}{cmcsc}{10 at #2pt}%
 \textfont\scfam=\csname sc#1\endcsname
 \fam\scfam\csname sc#1\endcsname}%
\rm }}
\makesize{Xf}{10}{VIIf}{7}{Vf}{5}{12pt}
\newfam\mibfam
\def\normalsize{\Xfsize
\def\sf{%
   \getf@nt{sf}{Xf}{cmss}{10}%
   \getf@nt{sf}{VIIf}{cmss}{10 at 7pt}%
   \getf@nt{sf}{Vf}{cmss}{10 at 5pt}%
   \textfont\sffam=\csname sfXf\endcsname
   \scriptfont\sffam=\csname sfVIIf\endcsname
   \scriptscriptfont\sffam=\csname sfVf\endcsname
   \fam\sffam\csname sfXf\endcsname}%
\def\mib{%
   \getf@nt{mib}{Xf}{cmmib}{10}%
   \getf@nt{mib}{VIIf}{cmmib}{10 at7pt}%
   \getf@nt{mib}{Vf}{cmmib}{10 at5pt}%
   \textfont\mibfam=\csname mibXf\endcsname
   \scriptfont\mibfam=\csname mibVIIf\endcsname
   \scriptscriptfont\mibfam=\csname mibVf\endcsname
   \fam\mibfam\csname mibXf\endcsname}%
\def\boldmath{\textfont1=\mibXf \scriptfont1=\mibVIIf
\scriptscriptfont1=\mibVf}%
\if Y\REFEREE \normalbaselineskip=2\normalbaselineskip
\normallineskip=0.1\normalbaselineskip\normalbaselines
\fi
\rm}
\Xfsize
\it\bf\tt\rm
\def\tenrm{\rmXf}
\def\fiverm{\rmVf}
\def\teni{\miXf}
\def\fivei{\miVf}
\def\tensy{\syXf}
\def\fivesy{\syVf}
\def\tenbf{\bfXf}
\def\fivebf{\bfVf}
\def\tentt{\ttXf}
\def\tensl{\slXf}
\def\tenit{\itXf}
\let\REFEREE=N
\normalsize
\it\bf\tt\sf\mib\rm
\catcode`@=12 % reset catcode
% This is layout.aa
% it sets up some measures and defines miscellaneous macros
\newdimen\fullhsize
\newcount\verybad \verybad=1010
\let\lr=L%
\baselineskip=12pt
\vsize=56\baselineskip
\hoffset=-1true cm
\voffset=-1true cm
\fullhsize=180mm
\newdimen\halfsize
\halfsize=88mm
\hsize=\halfsize
\def\fullline{\hbox to\fullhsize}
\def\makefootline{\baselineskip=12pt \fullline{\the\footline}}
\def\makeheadline{\vbox to 0pt{\vskip-22.5pt
            \fullline{\vbox to 8.5pt{}\the\headline}\vss}\nointerlineskip}
\hfuzz=2pt
\vfuzz=2pt
\tolerance=1000
\abovedisplayskip=3 mm plus6pt minus 4pt
\belowdisplayskip=3 mm plus6pt minus 4pt
\abovedisplayshortskip=0mm plus6pt
\belowdisplayshortskip=2 mm plus4pt minus 4pt
\parindent=1.5em
\newdimen\stdparindent\stdparindent\parindent
\frenchspacing
% Paginierung
\nopagenumbers
%
\predisplaypenalty=600        % Make a page break before a display harder
\displaywidowpenalty=2000     % and even harder for a widow display.
%
\def\widowsandclubs#1{\global\verybad=#1
   \global\widowpenalty=\the\verybad1      % default: 10101
   \global\clubpenalty=\the\verybad2  }    % default: 10102
\widowsandclubs{1010}
% This is runhead.aa
% it sets up the page layout for the first page of an article
% and enables the running head and its changing mechanism
%
\catcode`@=11 % use @ as a normal character
\let\firstpage=Y%
\def\paglay{\headline={\normalsize
\ifx Y\firstpage
 \global\let\firstpage=N%
 \let\REFEREE=N%
 \vbox{\hsize=.75\fullhsize
       \hrule
       \line{\vrule\kern3pt
             \vbox{\kern3pt
                   \hbox{\bf A\&A manuscript no.}
                   \hbox{(will be inserted by hand later)}
                   \kern3pt
                   \hrule
                   \kern3pt
                   \hbox{\bf Your thesaurus codes are:}
                   \hbox{\rightskip=0pt plus3em\advance\hsize by-7pt
                         \vbox{\bf\noindent\ignorespaces\the\THESAURUS}}%
                   \kern3pt}%
             \hfil
             \kern3pt
             \vrule}%
       \hrule}%
 \hfil\llap{\AALogo}%
\else
   \koltitle
\fi}}
\def\koltest{\setbox0=\hbox{\qquad\koltext}%
   \ifdim\wd0>\fullhsize
      \infuser{^^JThe running head built automatically from
               \string\AUTHOR\space and \string\MAINTITLE
               ^^Jexceeds the pagewidth, supply a shorter form
               using \string\AUTHORRUNNINGHEAD\string{...\string}
               ^^Jand/or \string\MAINTITLERUNNINGHEAD\string{...\string}
               after the \string\maketitle-command.}%
      \global\AUTHOR={Please give a shorter version with}%
      \global\MAINTITLE={{\tt\string\AUTHORRUNNINGHEAD\ }and/or%
                         {\tt\ \string\MAINTITLERUNNINGHEAD}}%
   \fi
   \global\let\kolTest=\relax}
%
\let\kolTest=\koltest
%
{\catcode`@=\active
\gdef\koltitle{%
   \petit
   \catcode`\@=\active
   \def@##1{}%
   \def\FOOTNOTE##1{}%
   \kolTest
   \ifodd\pageno
      \hfil\enspace
      \koltext
      \enspace\hfil\llap{\folio}%
   \else
      \rlap{\folio}%
      \hfil\enspace
      \koltext
      \enspace\hfil
   \fi}}
\def\koltext{\ignorespaces\the\AUTHOR\unskip: \ignorespaces
\the\MAINTITLE\unskip}
%
\def\kolTEST{\setbox0=\hbox{\qquad\koltext}%
   \ifdim\wd0>\fullhsize
      \infuser{^^JThe running head you supplied with
               \string\AUTHORRUNNINGHEAD\space and/or
               ^^J\string\MAINTITLERUNNINGHEAD\space exceeds the
               pagewidth, give a shorter form
               ^^Jusing \string\AUTHORRUNNINGHEAD\string{...\string}
               and/or \string\MAINTITLERUNNINGHEAD\string{...\string}
               ^^Jafter the \string\maketitle-command.}%
      \global\AUTHOR={Please give a shorter running head with}%
      \global\MAINTITLE={{\tt\string\AUTHORRUNNINGHEAD\ }and/or%
                         {\tt\ \string\MAINTITLERUNNINGHEAD}}%
   \fi
   \global\let\kolTest=\relax}
%
\def\MAINTITLERUNNINGHEAD#1{\global\MAINTITLE={#1}%
\infuser{^^JMAINTITLE part of running head has been changed}%
\let\kolTest=\kolTEST}
\def\AUTHORRUNNINGHEAD#1{\global\AUTHOR={#1}%
\infuser{^^JAUTHOR part of running head has been changed}%
\let\kolTest=\kolTEST}
\catcode`@=12 % reset catcode
% This is aacpetit.aa
% here the small print is defined
\catcode`@=11    % use @ as a normal character
\makesize{IXf}{9}{VIf}{6}{Vf}{5}{11pt}
\IXfsize\it\bf\tt\rm
\normalsize
\def\petit{\IXfsize
   \def\sf{%
      \getf@nt{sf}{IXf}{cmss}{9}%
      \getf@nt{sf}{VIf}{cmss}{10 at 6pt}%
      \getf@nt{sf}{Vf}{cmss}{10 at 5pt}%
      \textfont\sffam=\csname sfIXf\endcsname
      \scriptfont\sffam=\csname sfVIf\endcsname
      \scriptscriptfont\sffam=\csname sfVf\endcsname
      \fam\sffam\csname sfIXf\endcsname
}%
\def\mib{%
   \getf@nt{mib}{IXf}{cmmib}{10 at 9pt}%
   \getf@nt{mib}{VIf}{cmmib}{10 at 6pt}%
   \getf@nt{mib}{Vf}{cmmib}{10 at 5pt}%
   \textfont\mibfam=\csname mibIXf\endcsname
   \scriptfont\mibfam=\csname mibVIf\endcsname
   \scriptscriptfont\mibfam=\csname mibVf\endcsname
   \fam\mibfam\csname mibIXf\endcsname}%
\def\boldmath{\textfont1=\mibIXf\scriptfont1=\mibVIf
\scriptscriptfont1=\mibVf}%
 \if Y\REFEREE \normalbaselineskip=2\normalbaselineskip
 \normallineskip=0.1\normalbaselineskip\fi
 \setbox\strutbox=\hbox{\vrule height9pt depth2pt width0pt}%
 \normalbaselines\rm}%
%--------------------------------------------------------------------
\def\begpet{\vskip\petitsurround
\bgroup\petit}%  Beginn eines Paragraphen in petit
\def\endpet{\vskip\petitsurround
\egroup}%  Ende eines Paragraphen in petit
\petit\sf\mib
\normalsize
\catcode`@=12 % reset catcode
% This is aacmfont.aa
% It defines the fonts used for the cm version of the a&a package
% and connects the names to fonts already defined
%
% Fonts for \MAINTITLE
 \font \tamt            = cmmib10 scaled \magstep3
 \font \tams            = cmmib10 scaled \magstep1
%\font \tamss           = cmmib10  = \mibXf
 \let  \tamss=\mibXf
 \font \tast            = cmsy10 scaled \magstep3
 \font \tass            = cmsy10 scaled \magstep1
%\font \tasss           = cmsy10   = \syXf
 \let  \tasss=\syXf
 \font \tatt            = cmbx10 scaled \magstep3
 \font \tats            = cmbx10 scaled \magstep1
%\font \tatss           = cmbx10   = \bfXf
 \let  \tatss=\bfXf
% Fonts for \SUBTITLE
 \font \tbmt            = cmmib10 scaled \magstep2
%\font \tbms            = cmmib10  = \mibXf
 \let  \tbms=\mibXf
%\font \tbmss           = cmmib10 at 9pt = \mibIXf
 \let  \tbmss=\mibIXf
 \font \tbst            = cmsy10 scaled \magstep2
%\font \tbss            = cmsy10   = \syXf
 \let  \tbss=\syXf
%\font \tbsss           = cmsy9    = \syIXf
 \let  \tbsss=\syIXf
 \font \tbtt            = cmbx10 scaled \magstep2
%\font \tbts            = cmbx10   = \bfXf
 \let  \tbts=\bfXf
%\font \tbtss           = cmbx9    = \bfIXf
 \let  \tbtss=\bfIXf
 \font \headnotefont    = cmti10 scaled \magstep3
% This is ucgreek.aa
% the definition of versal greek characters
\mathchardef\Gamma  ="0000
\mathchardef\Delta  ="0001
\mathchardef\Theta  ="0002
\mathchardef\Lambda ="0003
\mathchardef\Xi     ="0004
\mathchardef\Pi     ="0005
\mathchardef\Sigma  ="0006
\mathchardef\Upsilon="0007
\mathchardef\Phi    ="0008
\mathchardef\Psi    ="0009
\mathchardef\Omega  ="000A
% This is aamisc.tex
% here miscellaneous macros are defined
%
% Makros to communicate with the user
\catcode`@=11 % use @ as a normal character
\newwrite\@info
\def\infuser#1{\immediate\write\@info{#1}}
\catcode`@=12 % at signs are no longer letters
%
\newlinechar=`\^^J % Zeilenumbruchhilfe fuer TeX-Meldungen am Bildschirm
\def\newline{\hfill\break}% makes a new line in the text :)
%-------------------------------------------------------------------
% draws a frame of height #1 cm times \hsize
\def\rahmen#1{\vbox{\hrule\line{\vrule\vbox to#1true
cm{\vfil}\hfil\vrule}\vfil\hrule}}
%-------------------------------------------------------------------
% shortcuts
\let\ts=\thinspace
\def\,{\relax\ifmmode\mskip\thinmuskip\else\thinspace\fi}
%-------------------------------------------------------------------
\def\unvskip{%
   \ifvmode
      \ifdim\lastskip=0pt
      \else
         \vskip-\lastskip
      \fi
   \fi}
% This is fleqn.tex
% it convinces TeX not to center the displayed formulas
\catcode`@=11    % use @ as a normal character
%
% allocate token registers for the equation and its number
\newtoks\eq\newtoks\eqn
%
% the horizontal size for a displayed formula is the actual \hsize
% minus the indention of the formula depending on the package
\newdimen\mathhsize
\def\calcmathhsize{\mathhsize=\hsize
\advance\mathhsize by-\mathindent}
\calcmathhsize
%
% define \eqalign@new, \displaylines@new, \(l)eqalignno@new to use this
% size but remember the old macros to make switching possible
\let\eqalign@old=\eqalign
\let\displaylines@old=\displaylines
\let\eqalignno@old=\eqalignno
\let\leqalignno@old=\leqalignno
\def\eqalign@new#1{\null\vcenter{\openup\jot\m@th
  \ialign{\strut\hfil$\displaystyle{##}$&$\displaystyle{{}##}$\hfil
      \crcr#1\crcr}}}
\def\displaylines@new#1{{}$\displ@y
\hbox{\vbox{\halign{$\@lign\hfil\displaystyle##\hfil$\crcr
    #1\crcr}}}${}}
\def\eqalignno@new#1{{}$\displ@y
  \hbox{\vbox{\halign
to\mathhsize{\hfil$\@lign\displaystyle{##}$\tabskip\z@skip
    &$\@lign\displaystyle{{}##}$\hfil\tabskip\centering
    &\llap{$\@lign##$}\tabskip\z@skip\crcr
    #1\crcr}}}${}}
\def\leqalignno@new#1{{}$\displ@y
\hbox{\vbox{\halign
to\mathhsize{\qquad\hfil$\@lign\displaystyle{##}$\tabskip\z@skip
    &$\@lign\displaystyle{{}##}$\hfil\tabskip\centering
    &\kern-\mathhsize\rlap{$\@lign##$}\tabskip\hsize\crcr
    #1\crcr}}}${}}
% main macro borrowed from the dirty tricks of the TeXbook
\def\generaldisplay{%
\ifeqno
       \ifleqno\leftline{$\displaystyle\the\eqn\quad\the\eq$}%
       \else\noindent\kern\mathindent\hbox to\mathhsize{$\displaystyle
             \the\eq\hfill\the\eqn$}%
       \fi
\else
       \kern\mathindent
       \hbox to\mathhsize{$\displaystyle\the\eq$\hss}%
\fi
\global\eq={}\global\eqn={}}%
%
% flags and defaults
\newif\ifeqno\newif\ifleqno
% check for the "$$"s
\def\displaysetup#1$${\displaytest#1\eqno\eqno\displaytest}
% look for equation numbers
\def\displaytest#1\eqno#2\eqno#3\displaytest{%
\if!#3!\ldisplaytest#1\leqno\leqno\ldisplaytest
\else\eqnotrue\leqnofalse\eqn={#2}\eq={#1}\fi
\generaldisplay$$}
\def\ldisplaytest#1\leqno#2\leqno#3\ldisplaytest{\eq={#1}%
\if!#3!\eqnofalse\else\eqnotrue\leqnotrue\eqn={#2}\fi}
%
% establish a switching between normal and flush left equations
%
\def\flushleftequations{%
   \infuser{^^JEquations are \ifx\Initexing\undefined now \fi
            typeset flush left.}%
   \everydisplay={\displaysetup}%
   \let\eqalign=\eqalign@new
   \let\displaylines=\displaylines@new
   \let\eqalignno=\eqalignno@new
   \let\leqalignno=\leqalignno@new}
%
\def\centeredequations{%
   \infuser{^^JEquations are \ifx\Initexing\undefined now \fi
            centered.}%
   \everydisplay={}%
   \let\eqalign=\eqalign@old
   \let\displaylines=\displaylines@old
   \let\eqalignno=\eqalignno@old
   \let\leqalignno=\leqalignno@old}
%
% set the default to flush left equations
\flushleftequations
%
\catcode`@=12 % at signs are no longer letters
% This is autnum.tex
% it defines a macro that steps and typesets a counter for equations
\newcount\eqnum\eqnum=0% register
%
% use: $$<formula>\eqno\autnum$$
%  or: $$\eqalignno{a&=b&\autnum\cr}$$
\def\autnum{\global\advance\eqnum by 1\relax{\rm(\the\eqnum)}}
% This is item.tex
% is defines a new \litem(item) with a left aligned argument
% and redefines plain \item(item)
%
\catcode`@=11    % use @ as a normal character
\def\litem#1{\item{#1\hfill}}
%
% \ch@ckitem(item)mark measures the width of the \item(item)s mark
% and issues a warning if it will not fit in the space provided
\def\ch@ckitemmark#1{\setbox0=\hbox{\enspace#1}%
\ifdim\wd0>\itemindent
   \infuser{^^J\string\item: Your mark `\string#1' is too wide. }%
\fi}
\def\ch@ckitemitemmark#1{\setbox0=\hbox{\kern\itemindent\enspace#1}%
\ifdim\wd0>\itemitemindent
   \infuser{^^J\string\itemitem: Your mark `\string#1' is too wide. }%
\fi}
%
% \set@item@mark is used to produce the \item's mark
\def\set@item@mark#1{\ch@ckitemmark{#1}%
\hbox to\itemindent{#1\hss}\ignorespaces}
% \set@itemitem@mark is used to produce the \itemitem's mark
\def\set@itemitem@mark#1{\ch@ckitemitemmark{#1}%
\dimen0=\itemitemindent
\advance\dimen0 by-\itemindent
\kern\itemindent\hbox to\dimen0{#1\hss}\ignorespaces}
%
% \setitem(item)indent takes its argument as the widest mark
% of an \item(item) and changes the \item(item)indent accordingly
\def\setitemindent#1{\setbox0=\hbox{\ignorespaces#1\unskip\enspace}%
\itemindent=\wd0\relax
\ifx\quiet\undefined
\infuser{^^J\string\setitemindent: Mark width modified to hold
         ^^J`\string#1' plus an \string\enspace\space gap. }%
\fi
}
\def\setitemitemindent#1{\setbox0=\hbox{\ignorespaces#1\unskip\enspace}%
\itemitemindent=\wd0\relax
\ifx\quiet\undefined
\infuser{^^J\string\setitemitemindent: Mark width modified to hold
         ^^J`\string#1' plus an \string\enspace\space gap. }%
\fi
\advance\itemitemindent by\itemindent}
%
% \item is redefined to produce a right aligned mark with
% a fixed gap, the hanging indentation has the width \itemindent.
% \itemitem is redefined to produce a left aligned mark with indention
% \itemindent, the hanging indentation has the width \itemitemindent.
% If there are flush left equations (\mathhsize is defined)
% that size is also corrected for use inside an \item(item).
\ifx\undefined\mathhsize
   \def\item{\par\noindent
   \hangindent\itemindent\hangafter=1\relax
   \set@item@mark}
   %
   \def\itemitem{\par\noindent
   \hangindent\itemitemindent\hangafter=1\relax
   \set@itemitem@mark}
\else
   \def\item{\par\noindent\advance\mathhsize by-\itemindent
   \hangindent\itemindent\hangafter=1\relax
   \everypar={\global\mathhsize=\hsize
   \global\advance\mathhsize by-\mathindent
   \global\everypar={}}\set@item@mark}
   %
   \def\itemitem{\par\noindent\advance\mathhsize by-\itemitemindent
   \hangindent\itemitemindent\hangafter=1\relax
   \everypar={\global\mathhsize=\hsize
   \global\advance\mathhsize by-\mathindent
   \global\everypar={}}\set@itemitem@mark}
\fi
\catcode`@=12 % at signs are no longer letters
% This is aatypset.tex
% it defines the final actions of the macro package
% i.e. printing of the identifying message and the
% characters invented by the author
\catcode`@=11    % use @ as a normal character
\newcount\the@end \global\the@end=0
\newbox\springer@macro \setbox\springer@macro=\vbox{}
\def\typeset{\setbox\springer@macro=\vbox{\begpet\noindent
   This article was processed by the author using
   Sprin\-ger-Ver\-lag \TeX{} A\&A macro package 1992.\par
   \egroup}\global\the@end=1}
% \show@special lists the contents of the (user defined) control
% sequence "specialn" where n is the lowercase roman numeral
% representation of the counter \footcount and then steps that counter.
\def\show@special{%
   \smallskip
   \noindent special character \#\number\sterne:
   \csname special\romannumeral\sterne\endcsname
   \advance\sterne by 1\relax
   \testspeci@l}
%
% \testspeci@l checks whether the control sequence "specialn" is
% defined, causing to print it and recursing to n+1 if yes,
% and aborting otherwise.
\def\testspeci@l{%
   \expandafter
   \ifx
      \csname special\romannumeral\sterne\endcsname
      \relax
      \let\next\relax
   \else
      \let\next\show@special
   \fi
   \next}
%
\outer\def\bye{\bigskip\typeset
\sterne=1 \testspeci@l
\if R\lr\null\fi\vfill\supereject\end}
\catcode`@=12    % reset catcode
% This is aalogo.tex
% it defines the A&A logo for the first page of an article
\def\AALogo{\setbox254=\hbox{ ASTROPHYSICS }%
\vbox{\baselineskip=10pt\hrule\hbox{\vrule\vbox{\kern3pt
\hbox to\wd254{\hfil ASTRONOMY\hfil}
\hbox to\wd254{\hfil AND\hfil}\copy254
\hbox to\wd254{\hfil\number\day.\number\month.\number\year\hfil}
\kern3pt}\vrule}\hrule}}
% This is aalegend.tex
% it defines the macro to produce figure captions
\def\figure#1#2{\medskip\noindent{\petit{\bf Fig.\ts#1.\
}\ignorespaces#2\par}}
% This is tabcap.tex
% it defines the macro to produce the table heads
% Tabellenkoepfe
\def\tabcap#1#2{\smallskip\noindent{\bf Table\ts\ignorespaces
#1\unskip.\ }\ignorespaces #2\vskip3mm}
% This is counters.tex
% it defines and initializes the counters needed
\catcode`@=11    % use @ as a normal character
\expandafter \newcount \csname c@Tl\endcsname
    \csname c@Tl\endcsname=0
\expandafter \newcount \csname c@Tm\endcsname
    \csname c@Tm\endcsname=0
\expandafter \newcount \csname c@Tn\endcsname
    \csname c@Tn\endcsname=0
\expandafter \newcount \csname c@To\endcsname
    \csname c@To\endcsname=0
\expandafter \newcount \csname c@Tp\endcsname
    \csname c@Tp\endcsname=0
\expandafter \newcount \csname c@fn\endcsname
    \csname c@fn\endcsname=0
\def \stepc#1    {\global
    \expandafter
    \advance
    \csname c@#1\endcsname by 1}
\def \resetcount#1    {\global
    \csname c@#1\endcsname=0}
\def\@nameuse#1{\csname #1\endcsname}
\def\arabic#1{\@arabic{\@nameuse{c@#1}}}
\def\@arabic#1{\ifnum #1>0 \number #1\fi}
\catcode`@=12    % reset catcode
% This is maintitl.aa
% it defines the macros to start and end the main title
\catcode`@=11 % use @ as a normal character
\def \aTa  { \goodbreak
\bgroup
\par
\let\bf=\relax\let\boldmath=\relax\let\bffam=\z@
\textfont0=\tatt \scriptfont0=\tats \scriptscriptfont0=\tatss
\textfont1=\tamt \scriptfont1=\tams \scriptscriptfont1=\tamss
\textfont2=\tast \scriptfont2=\tass \scriptscriptfont2=\tasss
\ifx\grfam\undefined\else
   \textfont\grfam=\tagrt \scriptfont\grfam=\tagrs
   \scriptscriptfont\grfam=\tagrss
\fi
\baselineskip=\tabaselineskip
\lineskiplimit=0pt\lineskip=0pt
\rightskip=0pt plus4cm
\pretolerance=10000
\noindent
\tatt}
% --------------------------------------------------------------
% Ende Ueberschrift
%
\def\eTa{\vskip10pt\egroup
         \noindent
         \ignorespaces}
\catcode`@=12 % at signs are no longer letters
% This is subtitl.tex
% it defines the macros to start and end the subtitle
\catcode`@=11 % use @ as a normal character
\def\aTb{\goodbreak
\bgroup
\par
\let\bf=\relax\let\boldmath=\relax\let\bffam=\z@
\textfont0=\tbtt \scriptfont0=\tbts \scriptscriptfont0=\tbtss
\textfont1=\tbmt \scriptfont1=\tbms \scriptscriptfont1=\tbmss
\textfont2=\tbst \scriptfont2=\tbss \scriptscriptfont2=\tbsss
\ifx\grfam\undefined\else
   \textfont\grfam=\tbgrt \scriptfont\grfam=\tbgrs
   \scriptscriptfont\grfam=\tbgrss
\fi
\baselineskip=\tbbaselineskip
\lineskip=0pt\lineskiplimit=0pt
\rightskip=0pt plus4cm
\pretolerance=10000
\noindent
\tbtt}
% ---------------------------------------------------------------
% Ende Ueberschrift 2. Ordnung
%
\def\eTb{\vskip10pt
    \egroup
    \noindent
    \ignorespaces}
\catcode`@=12 % at signs are no longer letters
% This is aatita.tex
% it defines the heading of first order that is numbered automatically
\catcode`@=11    % use @ as a normal character
\newcount\section@penalty  \section@penalty=0
\newcount\subsection@penalty  \subsection@penalty=0
\newcount\subsubsection@penalty  \subsubsection@penalty=0
%
\def\titlea#1{\par\stepc{Tl}
    \resetcount{Tm}
    \bgroup
       \normalsize
       \bf \rightskip 0pt plus4em
       \pretolerance=20000
       \boldmath
       \setbox0=\vbox{\vskip\tabefore
          \noindent
          \arabic{Tl}.\
          \ignorespaces#1
          \vskip\taafter}
       \dimen0=\ht0\advance\dimen0 by\dp0
       \advance\dimen0 by 2\baselineskip
       \advance\dimen0 by\pagetotal
       \ifdim\dimen0>\pagegoal
          \ifdim\pagetotal>\pagegoal
          \else\eject\fi\fi
       \vskip\tabefore
       \penalty\section@penalty \global\section@penalty=-200
       \global\subsection@penalty=10007
       \noindent
       \arabic{Tl}.\
       \ignorespaces#1\par
    \egroup
    \nobreak
    \vskip\taafter
    \parindent=0pt
    \let\lasttitle=A%
\everypar={\parindent=\stdparindent
    \penalty\z@\let\lasttitle=N\everypar={}}%
    \ignorespaces}
\catcode`@=12    % reset catcode
% This is aatitb.tex
% it defines the heading of second order that is numbered automatically
\catcode`@=11    % use @ as a normal character
\def\titleb#1{\par\stepc{Tm}
    \resetcount{Tn}
    \if N\lasttitle\else\vskip\tbbeforeback\fi
    \bgroup
       \normalsize
       \raggedright
       \pretolerance=10000
       \it
       \setbox0=\vbox{\vskip\tbbefore
          \normalsize
          \raggedright
          \pretolerance=10000
          \noindent \it \arabic{Tl}.\arabic{Tm}.\ \ignorespaces#1
          \vskip\tbafter}
       \dimen0=\ht0\advance\dimen0 by\dp0\advance\dimen0 by 2\baselineskip
       \advance\dimen0 by\pagetotal
       \ifdim\dimen0>\pagegoal
          \ifdim\pagetotal>\pagegoal
          \else \if N\lasttitle\eject\fi \fi\fi
       \vskip\tbbefore
       \if N\lasttitle \penalty\subsection@penalty \fi
       \global\subsection@penalty=-100
       \global\subsubsection@penalty=10007
       \noindent \arabic{Tl}.\arabic{Tm}.\ \ignorespaces#1\par
    \egroup
    \nobreak
    \vskip\tbafter
    \let\lasttitle=B%
    \parindent=0pt
    \everypar={\parindent=\stdparindent
       \penalty\z@\let\lasttitle=N\everypar={}}%
       \ignorespaces}
\catcode`@=12    % reset catcode
% This is aatitc.tex
% it defines the heading of third order that is numbered automatically
\catcode`@=11    % use @ as a normal character
\def\titlec#1{\par\stepc{Tn}
    \resetcount{To}
    \if N\lasttitle\else\vskip\tcbeforeback\fi
    \bgroup
       \normalsize
       \raggedright
       \pretolerance=10000
       \setbox0=\vbox{\vskip\tcbefore
          \noindent
          \arabic{Tl}.\arabic{Tm}.\arabic{Tn}.\
          \ignorespaces#1\vskip\tcafter}
       \dimen0=\ht0\advance\dimen0 by\dp0\advance\dimen0 by 2\baselineskip
       \advance\dimen0 by\pagetotal
       \ifdim\dimen0>\pagegoal
           \ifdim\pagetotal>\pagegoal
           \else \if N\lasttitle\eject\fi \fi\fi
       \vskip\tcbefore
       \if N\lasttitle \penalty\subsubsection@penalty \fi
       \global\subsubsection@penalty=-50
       \noindent
       \arabic{Tl}.\arabic{Tm}.\arabic{Tn}.\
       \ignorespaces#1\par
    \egroup
    \nobreak
    \vskip\tcafter
    \let\lasttitle=C%
    \parindent=0pt
    \everypar={\parindent=\stdparindent
       \penalty\z@\let\lasttitle=N\everypar={}}%
       \ignorespaces}
\catcode`@=12    % reset catcode
% This is aatitd.tex
% it defines the heading of fourth order that is numbered automatically
\def\titled#1{\par\stepc{To}
    \resetcount{Tp}
    \if N\lasttitle\else\vskip\tdbeforeback\fi
    \vskip\tdbefore
    \bgroup
       \normalsize
       \if N\lasttitle \penalty-50 \fi
       \it \noindent \ignorespaces#1\unskip\
    \egroup\ignorespaces}
% This is referenc.tex
% it defines the macros needed to produce the references
%
\def\begref#1{\par
   \unvskip
   \goodbreak\vskip\tabefore
   {\noindent\bf\ignorespaces#1%
   \par\vskip\taafter}\nobreak\let\INS=N}
\def\ref{\if N\INS\let\INS=Y\else\goodbreak\fi
   \hangindent\stdparindent\hangafter=1\noindent\ignorespaces}
\def\endref{\goodbreak}% Ende der Referenzen
% This is acknow.tex
% it prints the acknowledgement text
\def\acknow#1{\par
   \unvskip
   \vskip\tcbefore
   \noindent{\it Acknowledgements\/}. %
   \ignorespaces#1\par
   \vskip\tcafter}
% This is appendix.aa
% it starts an appendix section without automatic numeration
\def\appendix#1{\vskip\tabefore
    \vbox{\noindent{\bf Appendix #1}\vskip\taafter}%
    \global\eqnum=0\relax
    \nobreak\noindent\ignorespaces}
% This is referee.tex
% it allows the author to produce a referees copy
% single column wider line spacing
\newbox\refereebox
\setbox\refereebox=\vbox
to0pt{\vskip0.5cm\fullline{\hrulefill\tentt\lower0.5ex
\hbox{\kern5pt referee's copy\kern5pt}\hrulefill}\vss}%
\def\refereelayout{\let\REFEREE=Y\footline={\copy\refereebox}%
    \infuser{^^JA referee's copy will be produced}\par
    \if N\lr\else\onecolumn\topskip=10pt\fi
    \normalsize
    \calcmathhsize}
% This is symbols.tex
% the symbols not available in plain TeX are constructed
% by overprinting some characters
\def\sun{\hbox{$\odot$}}
\def\la{\mathrel{\mathchoice {\vcenter{\offinterlineskip\halign{\hfil
$\displaystyle##$\hfil\cr<\cr\noalign{\vskip1.5pt}\sim\cr}}}
{\vcenter{\offinterlineskip\halign{\hfil$\textstyle##$\hfil\cr<\cr
\noalign{\vskip1.0pt}\sim\cr}}}
{\vcenter{\offinterlineskip\halign{\hfil$\scriptstyle##$\hfil\cr<\cr
\noalign{\vskip0.5pt}\sim\cr}}}
{\vcenter{\offinterlineskip\halign{\hfil$\scriptscriptstyle##$\hfil
\cr<\cr\noalign{\vskip0.5pt}\sim\cr}}}}}
\def\ga{\mathrel{\mathchoice {\vcenter{\offinterlineskip\halign{\hfil
$\displaystyle##$\hfil\cr>\cr\noalign{\vskip1.5pt}\sim\cr}}}
{\vcenter{\offinterlineskip\halign{\hfil$\textstyle##$\hfil\cr>\cr
\noalign{\vskip1.0pt}\sim\cr}}}
{\vcenter{\offinterlineskip\halign{\hfil$\scriptstyle##$\hfil\cr>\cr
\noalign{\vskip0.5pt}\sim\cr}}}
{\vcenter{\offinterlineskip\halign{\hfil$\scriptscriptstyle##$\hfil
\cr>\cr\noalign{\vskip0.5pt}\sim\cr}}}}}
\def\sq{\hbox{\rlap{$\sqcap$}$\sqcup$}}
\def\degr{\hbox{$^\circ$}}
\def\arcmin{\hbox{$^\prime$}}
\def\arcsec{\hbox{$^{\prime\prime}$}}
\def\utw{\smash{\rlap{\lower5pt\hbox{$\sim$}}}}
\def\udtw{\smash{\rlap{\lower6pt\hbox{$\approx$}}}}
\def\fd{\hbox{$.\!\!^{\rm d}$}}
\def\fh{\hbox{$.\!\!^{\rm h}$}}
\def\fm{\hbox{$.\!\!^{\rm m}$}}
\def\fs{\hbox{$.\!\!^{\rm s}$}}
\def\fdg{\hbox{$.\!\!^\circ$}}
\def\farcm{\hbox{$.\mkern-4mu^\prime$}}
\def\farcs{\hbox{$.\!\!^{\prime\prime}$}}
\def\fp{\hbox{$.\!\!^{\scriptscriptstyle\rm p}$}}
\def\getsto{\mathrel{\mathchoice {\vcenter{\offinterlineskip
\halign{\hfil$\displaystyle##$\hfil\cr\gets\cr\to\cr}}}
{\vcenter{\offinterlineskip\halign{\hfil$\textstyle##$\hfil\cr
\gets\cr\to\cr}}}
{\vcenter{\offinterlineskip\halign{\hfil$\scriptstyle##$\hfil\cr
\gets\cr\to\cr}}}
{\vcenter{\offinterlineskip\halign{\hfil$\scriptscriptstyle##$\hfil\cr
\gets\cr\to\cr}}}}}
\def\cor{\mathrel{\mathchoice {\hbox{$\widehat=$}}{\hbox{$\widehat=$}}
{\hbox{$\scriptstyle\hat=$}}
{\hbox{$\scriptscriptstyle\hat=$}}}}
\def\lid{\mathrel{\mathchoice {\vcenter{\offinterlineskip\halign{\hfil
$\displaystyle##$\hfil\cr<\cr\noalign{\vskip1.5pt}=\cr}}}
{\vcenter{\offinterlineskip\halign{\hfil$\textstyle##$\hfil\cr<\cr
\noalign{\vskip1pt}=\cr}}}
{\vcenter{\offinterlineskip\halign{\hfil$\scriptstyle##$\hfil\cr<\cr
\noalign{\vskip0.5pt}=\cr}}}
{\vcenter{\offinterlineskip\halign{\hfil$\scriptscriptstyle##$\hfil\cr
<\cr\noalign{\vskip0.5pt}=\cr}}}}}
\def\gid{\mathrel{\mathchoice {\vcenter{\offinterlineskip\halign{\hfil
$\displaystyle##$\hfil\cr>\cr\noalign{\vskip1.5pt}=\cr}}}
{\vcenter{\offinterlineskip\halign{\hfil$\textstyle##$\hfil\cr>\cr
\noalign{\vskip1pt}=\cr}}}
{\vcenter{\offinterlineskip\halign{\hfil$\scriptstyle##$\hfil\cr>\cr
\noalign{\vskip0.5pt}=\cr}}}
{\vcenter{\offinterlineskip\halign{\hfil$\scriptscriptstyle##$\hfil\cr
>\cr\noalign{\vskip0.5pt}=\cr}}}}}
\def\sol{\mathrel{\mathchoice {\vcenter{\offinterlineskip\halign{\hfil
$\displaystyle##$\hfil\cr\sim\cr\noalign{\vskip-0.2mm}<\cr}}}
{\vcenter{\offinterlineskip
\halign{\hfil$\textstyle##$\hfil\cr\sim\cr<\cr}}}
{\vcenter{\offinterlineskip
\halign{\hfil$\scriptstyle##$\hfil\cr\sim\cr<\cr}}}
{\vcenter{\offinterlineskip
\halign{\hfil$\scriptscriptstyle##$\hfil\cr\sim\cr<\cr}}}}}
\def\sog{\mathrel{\mathchoice {\vcenter{\offinterlineskip\halign{\hfil
$\displaystyle##$\hfil\cr\sim\cr\noalign{\vskip-0.2mm}>\cr}}}
{\vcenter{\offinterlineskip
\halign{\hfil$\textstyle##$\hfil\cr\sim\cr>\cr}}}
{\vcenter{\offinterlineskip
\halign{\hfil$\scriptstyle##$\hfil\cr\sim\cr>\cr}}}
{\vcenter{\offinterlineskip
\halign{\hfil$\scriptscriptstyle##$\hfil\cr\sim\cr>\cr}}}}}
\def\lse{\mathrel{\mathchoice {\vcenter{\offinterlineskip\halign{\hfil
$\displaystyle##$\hfil\cr<\cr\noalign{\vskip1.5pt}\simeq\cr}}}
{\vcenter{\offinterlineskip\halign{\hfil$\textstyle##$\hfil\cr<\cr
\noalign{\vskip1pt}\simeq\cr}}}
{\vcenter{\offinterlineskip\halign{\hfil$\scriptstyle##$\hfil\cr<\cr
\noalign{\vskip0.5pt}\simeq\cr}}}
{\vcenter{\offinterlineskip
\halign{\hfil$\scriptscriptstyle##$\hfil\cr<\cr
\noalign{\vskip0.5pt}\simeq\cr}}}}}
\def\gse{\mathrel{\mathchoice {\vcenter{\offinterlineskip\halign{\hfil
$\displaystyle##$\hfil\cr>\cr\noalign{\vskip1.5pt}\simeq\cr}}}
{\vcenter{\offinterlineskip\halign{\hfil$\textstyle##$\hfil\cr>\cr
\noalign{\vskip1.0pt}\simeq\cr}}}
{\vcenter{\offinterlineskip\halign{\hfil$\scriptstyle##$\hfil\cr>\cr
\noalign{\vskip0.5pt}\simeq\cr}}}
{\vcenter{\offinterlineskip
\halign{\hfil$\scriptscriptstyle##$\hfil\cr>\cr
\noalign{\vskip0.5pt}\simeq\cr}}}}}
\def\grole{\mathrel{\mathchoice {\vcenter{\offinterlineskip\halign{\hfil
$\displaystyle##$\hfil\cr>\cr\noalign{\vskip-1.5pt}<\cr}}}
{\vcenter{\offinterlineskip\halign{\hfil$\textstyle##$\hfil\cr
>\cr\noalign{\vskip-1.5pt}<\cr}}}
{\vcenter{\offinterlineskip\halign{\hfil$\scriptstyle##$\hfil\cr
>\cr\noalign{\vskip-1pt}<\cr}}}
{\vcenter{\offinterlineskip\halign{\hfil$\scriptscriptstyle##$\hfil\cr
>\cr\noalign{\vskip-0.5pt}<\cr}}}}}
\def\leogr{\mathrel{\mathchoice {\vcenter{\offinterlineskip\halign{\hfil
$\displaystyle##$\hfil\cr<\cr\noalign{\vskip-1.5pt}>\cr}}}
{\vcenter{\offinterlineskip\halign{\hfil$\textstyle##$\hfil\cr
<\cr\noalign{\vskip-1.5pt}>\cr}}}
{\vcenter{\offinterlineskip\halign{\hfil$\scriptstyle##$\hfil\cr
<\cr\noalign{\vskip-1pt}>\cr}}}
{\vcenter{\offinterlineskip\halign{\hfil$\scriptscriptstyle##$\hfil\cr
<\cr\noalign{\vskip-0.5pt}>\cr}}}}}
\def\loa{\mathrel{\mathchoice {\vcenter{\offinterlineskip\halign{\hfil
$\displaystyle##$\hfil\cr<\cr\noalign{\vskip1.5pt}\approx\cr}}}
{\vcenter{\offinterlineskip\halign{\hfil$\textstyle##$\hfil\cr<\cr
\noalign{\vskip1.0pt}\approx\cr}}}
{\vcenter{\offinterlineskip\halign{\hfil$\scriptstyle##$\hfil\cr<\cr
\noalign{\vskip0.5pt}\approx\cr}}}
{\vcenter{\offinterlineskip\halign{\hfil$\scriptscriptstyle##$\hfil\cr
<\cr\noalign{\vskip0.5pt}\approx\cr}}}}}
\def\goa{\mathrel{\mathchoice {\vcenter{\offinterlineskip\halign{\hfil
$\displaystyle##$\hfil\cr>\cr\noalign{\vskip1.5pt}\approx\cr}}}
{\vcenter{\offinterlineskip\halign{\hfil$\textstyle##$\hfil\cr>\cr
\noalign{\vskip1.0pt}\approx\cr}}}
{\vcenter{\offinterlineskip\halign{\hfil$\scriptstyle##$\hfil\cr>\cr
\noalign{\vskip0.5pt}\approx\cr}}}
{\vcenter{\offinterlineskip\halign{\hfil$\scriptscriptstyle##$\hfil\cr
>\cr\noalign{\vskip0.5pt}\approx\cr}}}}}
\def\bbbr{{\rm I\!R}} %reelle Zahlen
\def\bbbn{{\rm I\!N}} %natuerliche Zahlen
\def\bbbm{{\rm I\!M}}
\def\bbbh{{\rm I\!H}}
\def\bbbf{{\rm I\!F}}
\def\bbbk{{\rm I\!K}}
\def\bbbp{{\rm I\!P}}
\def\bbbone{{\mathchoice {\rm 1\mskip-4mu l} {\rm 1\mskip-4mu l}
{\rm 1\mskip-4.5mu l} {\rm 1\mskip-5mu l}}}
\def\bbbc{{\mathchoice {\setbox0=\hbox{$\displaystyle\rm C$}\hbox{\hbox
to0pt{\kern0.4\wd0\vrule height0.9\ht0\hss}\box0}}
{\setbox0=\hbox{$\textstyle\rm C$}\hbox{\hbox
to0pt{\kern0.4\wd0\vrule height0.9\ht0\hss}\box0}}
{\setbox0=\hbox{$\scriptstyle\rm C$}\hbox{\hbox
to0pt{\kern0.4\wd0\vrule height0.9\ht0\hss}\box0}}
{\setbox0=\hbox{$\scriptscriptstyle\rm C$}\hbox{\hbox
to0pt{\kern0.4\wd0\vrule height0.9\ht0\hss}\box0}}}}
\def\bbbq{{\mathchoice {\setbox0=\hbox{$\displaystyle\rm Q$}\hbox{\raise
0.15\ht0\hbox to0pt{\kern0.4\wd0\vrule height0.8\ht0\hss}\box0}}
{\setbox0=\hbox{$\textstyle\rm Q$}\hbox{\raise
0.15\ht0\hbox to0pt{\kern0.4\wd0\vrule height0.8\ht0\hss}\box0}}
{\setbox0=\hbox{$\scriptstyle\rm Q$}\hbox{\raise
0.15\ht0\hbox to0pt{\kern0.4\wd0\vrule height0.7\ht0\hss}\box0}}
{\setbox0=\hbox{$\scriptscriptstyle\rm Q$}\hbox{\raise
0.15\ht0\hbox to0pt{\kern0.4\wd0\vrule height0.7\ht0\hss}\box0}}}}
\def\bbbt{{\mathchoice {\setbox0=\hbox{$\displaystyle\rm
T$}\hbox{\hbox to0pt{\kern0.3\wd0\vrule height0.9\ht0\hss}\box0}}
{\setbox0=\hbox{$\textstyle\rm T$}\hbox{\hbox
to0pt{\kern0.3\wd0\vrule height0.9\ht0\hss}\box0}}
{\setbox0=\hbox{$\scriptstyle\rm T$}\hbox{\hbox
to0pt{\kern0.3\wd0\vrule height0.9\ht0\hss}\box0}}
{\setbox0=\hbox{$\scriptscriptstyle\rm T$}\hbox{\hbox
to0pt{\kern0.3\wd0\vrule height0.9\ht0\hss}\box0}}}}
\def\bbbs{{\mathchoice
{\setbox0=\hbox{$\displaystyle     \rm S$}\hbox{\raise0.5\ht0\hbox
to0pt{\kern0.35\wd0\vrule height0.45\ht0\hss}\hbox
to0pt{\kern0.55\wd0\vrule height0.5\ht0\hss}\box0}}
{\setbox0=\hbox{$\textstyle        \rm S$}\hbox{\raise0.5\ht0\hbox
to0pt{\kern0.35\wd0\vrule height0.45\ht0\hss}\hbox
to0pt{\kern0.55\wd0\vrule height0.5\ht0\hss}\box0}}
{\setbox0=\hbox{$\scriptstyle      \rm S$}\hbox{\raise0.5\ht0\hbox
to0pt{\kern0.35\wd0\vrule height0.45\ht0\hss}\raise0.05\ht0\hbox
to0pt{\kern0.5\wd0\vrule height0.45\ht0\hss}\box0}}
{\setbox0=\hbox{$\scriptscriptstyle\rm S$}\hbox{\raise0.5\ht0\hbox
to0pt{\kern0.4\wd0\vrule height0.45\ht0\hss}\raise0.05\ht0\hbox
to0pt{\kern0.55\wd0\vrule height0.45\ht0\hss}\box0}}}}
\def\bbbz{{\mathchoice {\hbox{$\sf\textstyle Z\kern-0.4em Z$}}
{\hbox{$\sf\textstyle Z\kern-0.4em Z$}}
{\hbox{$\sf\scriptstyle Z\kern-0.3em Z$}}
{\hbox{$\sf\scriptscriptstyle Z\kern-0.2em Z$}}}}
\def\diameter{{\ifmmode\oslash\else$\oslash$\fi}}
%
% redefine \Re and \Im
\def\Re{{\rm Re}}
\def\Im{{\rm Im}}
%
\def\diff{{\rm d}}
\def\eul{{\rm e}}
\def\imag{{\rm i}}
% This is vec.tex
% it defines vectors in boldface math and tensors in sans serif style
%
\catcode`@=11 % use @ as a normal character
\def\vec#1{{\boldmath\bf
\textfont\z@=\textfont\bffam\scriptfont\z@=\scriptfont\bffam
\scriptscriptfont\z@=\scriptscriptfont\bffam
\ifmmode
\mathchoice{\hbox{$\displaystyle#1$}}{\hbox{$\textstyle#1$}}
{\hbox{$\scriptstyle#1$}}{\hbox{$\scriptscriptstyle#1$}}\else
$#1$\fi}}
%
\def\tens#1{\relax\ifmmode
\mathchoice{\hbox{$\displaystyle\sf#1$}}{\hbox{$\textstyle\sf#1$}}
{\hbox{$\scriptstyle\sf#1$}}{\hbox{$\scriptscriptstyle\sf#1$}}\else
$\sf#1$\fi}
\catcode`@=12 % at signs are no longer letters
% This is titsetup.tex
% it defines variables and macros for the title page
% Variablenvereinbarung fuer Titelseitenautomatik
\newcount\sterne \sterne=0
\newdimen\fullhead
{\catcode`@=11    % use @ as a normal character
\def\newtoks{\alloc@5\toks\toksdef\@cclvi}
\outer\gdef\makenewtoks#1{\newtoks#1#1={ ????? }}}
\makenewtoks\DATE
\makenewtoks\MAINTITLE
\makenewtoks\SUBTITLE
\makenewtoks\AUTHOR
\makenewtoks\INSTITUTE
\makenewtoks\ABSTRACT
\makenewtoks\KEYWORDS
\makenewtoks\THESAURUS
\makenewtoks\OFFPRINTS
\makenewtoks\HEADNOTE
% Klammeraffe(@-Zeichen) wird Schluesselbuchstabe fuer affiliations
% solange Titel-page aktiv ist (Benutzung in AUTHOR und INSTITUTE)
\let\INS=N%
{\catcode`\@=\active
% Aktionen, die bei Antreffen des @-Zeichens zu machen sind;
% zwei Faelle a) @ bei AUTHOR, b) @ bei INSTITUTE
\gdef@#1{%
\if N\INS
   $^{#1}$%
\else
   \let\INS=Y%
   \par
   \noindent\hbox to0.5\stdparindent{$^{#1}$\hfil}\ignorespaces
\fi}%
}% @ wieder normal
% Automatische Fussnotennumerierung mit wachsender Anzahl Sterne
\def\mehrsterne{\global\advance\sterne by1\relax}%
% This is footnote.tex
% it defines all footnote macros
\def\footnoterule{\kern-3pt\hrule width 2true cm\kern2.6pt}% Trennlinie
%-------------------------------------------------------------------------------
\def\makeOFFPRINTS#1{\bgroup\let\REFEREE=N \normalsize
       \if N\lr\hsize=\fullhsize\else\hsize=\halfsize\fi
       \lineskiplimit=0pt\lineskip=0pt
       \def\textindent##1{\noindent{\it Send offprint
          requests to\/}: }\relax
       \vfootnote{nix}{\ignorespaces#1}\egroup}
%-------------------------------------------------------------------------------
% Fussnote mit stern(*) gekennzeichnet
\def\makesterne{\count254=0\loop\ifnum\count254<\sterne
\advance\count254 by1\star\repeat}
\def\FOOTNOTE#1{\bgroup\let\REFEREE=N
       \ifhmode\unskip\fi
       \mehrsterne$^{\makesterne}$\relax
       \normalsize
       \if N\lr\hsize=\fullhsize\else\hsize=\halfsize\fi
       \lineskiplimit=0pt\lineskip=0pt
       \def\textindent##1{\noindent\hbox
       to\stdparindent{##1\hss}}\relax
       \vfootnote{$^{\makesterne}$}{\ignorespaces#1}\egroup}
%
\def\PRESADD#1{\FOOTNOTE{Present address: \ignorespaces#1}}
%
% Automatisch numerierte Fussnote
\def\fonote#1{\relax\ifhmode\unskip\fi
       \mehrsterne$^{\the\sterne}$\bgroup
       \normalsize
       \if N\lr\hsize=\fullhsize\else\hsize=\halfsize\fi
       \def\textindent##1{\noindent\hbox
       to\stdparindent{##1\hss}}\relax
       \vfootnote{$^{\the\sterne}$}{\ignorespaces#1}\egroup}
% This is maketitl.tex
% it defines all macros to construct the title page
%
\def\missmsg#1{\infuser{^^JMissing #1 }}
%% test if missing:
%
\def\tstmiss#1#2#3#4#5{%
\edef\test{\the #1}%
\ifx\test\missing%
  #2\relax%  infuser
  #3%   action if missing
\else
  \ifx\test\missingi%
    #2\relax%  infuser
    #3%   action if missing
  \else #4%  action if existing
  \fi
\fi
#5%   action at any rate
}%
\def\strich{\par
\vbox to0pt{\hrule width\hsize\vss}\vskip-1.2\baselineskip
\vskip0pt plus3\baselineskip\relax}%
%
\def\at{\char64 }
%
% Hauptmacro fuer automatische Titelseite
\def\maketitle{\paglay%
\def\missing{ ????? }% Schablone zur Erkennung von nicht ausgefuellten
\def\missingi{ }% Schablone zur Erkennung von nicht ausgefuellten
% Feldern
%
% Methode zum Test auf Leerfelder: Variable wird mit \missing=" ????? "
% verglichen; Fallunterscheidung.
% \edef\test{\the\VARIABLE} macht die Variable dem Vergleich zugaenglich
% \ifx\test = \missing    d.h. steht in Variable der Text: " ????? "?
% !!! Aktion fuer Fall ja, hier wurde also nichts eingetragen !!!
% \else !!! Fall fuer ausgefuellte Variable!!! \fi
{\parskip=0pt\relax
\setbox0=\vbox{\hsize=\fullhsize\null\vskip2truecm
%
\tstmiss%
  {\HEADNOTE}%
  {}%
  {}%
  {%   write HEADNOTE:
   \noindent{\headnotefont\ignorespaces\the\HEADNOTE}\vskip8mm
   }%
  {}%
%
\tstmiss%
  {\MAINTITLE}%
  {}%
  {\global\MAINTITLE={MAINTITLE should be given}}%
  {}%
  {%   write MAINTITLE:
   \aTa\ignorespaces\the\MAINTITLE\eTa}%
%
\tstmiss%
  {\SUBTITLE}%
  {}%
  {}%
  {%   write SUBTITLE:
   \aTb\ignorespaces\the\SUBTITLE\eTb}%
  {}%
%
\tstmiss%
  {\AUTHOR}%
  {}%
  {\AUTHOR={Name(s) and initial(s) of author(s) should be given}}
  {}%
  {%   write AUTHOR:
\noindent{\bf\ignorespaces\the\AUTHOR\vskip4pt}}%
%
\tstmiss%
  {\INSTITUTE}%
  {}%
  {\INSTITUTE={Address(es) of author(s) should be given.}}%
  {}%
  {%   write INSTITUTE:
   \let\INS=E
\noindent\ignorespaces\the\INSTITUTE\vskip10pt}%
%
\tstmiss%
  {\DATE}%
  {}%
  {\DATE={$[$the date of receipt and acceptance should be inserted
later$]$}}%
  {}%
  {%   write DATE:
{\noindent\ignorespaces\the\DATE\vskip21pt}\bf A}%
%
}%
%
\global\fullhead=\ht0\global\advance\fullhead by\dp0
\global\advance\fullhead by10pt\global\sterne=0
%
{\hsize=\halfsize\null\vskip2truecm
\tstmiss%
  {\OFFPRINTS}%
  {}%
  {}%
  {\makeOFFPRINTS{\the\OFFPRINTS}}%
  {}%
%
\hsize=\fullhsize
%
\tstmiss%
  {\HEADNOTE}%
  {}%
  {}%
  {%   write HEADNOTE:
   \noindent{\headnotefont\ignorespaces\the\HEADNOTE}\vskip8mm
   }%
  {}%
%
\tstmiss%
  {\MAINTITLE}%
  {\missmsg{MAINTITLE}}%
  {\global\MAINTITLE={MAINTITLE should be given}}%
  {}%
  {%   write MAINTITLE:
   \aTa\ignorespaces\the\MAINTITLE\eTa}%
%
\tstmiss%
  {\SUBTITLE}%
  {}%
  {}%
  {%   write SUBTITLE:
   \aTb\ignorespaces\the\SUBTITLE\eTb}%
  {}%
%
\tstmiss%
  {\AUTHOR}%
  {\missmsg{name(s) and initial(s) of author(s)}}%
  {\AUTHOR={Name(s) and initial(s) of author(s) should be given}}
  {}%
  {%   write AUTHOR:
\noindent{\bf\ignorespaces\the\AUTHOR\vskip4pt}}%
%
\tstmiss%
  {\INSTITUTE}%
  {\missmsg{address(es) of author(s)}}%
  {\INSTITUTE={Address(es) of author(s) should be given.}}%
  {}%
  {%   write INSTITUTE:
   \let\INS=E
\noindent\ignorespaces\the\INSTITUTE\vskip10pt}%
%
\tstmiss%
  {\DATE}%
  {\infuser{^^JThe date of receipt and acceptance should be inserted
later.}}%
  {\DATE={$[$the date of receipt and acceptance should be inserted
later$]$}}%
  {}%
  {%   write DATE:
{\noindent\ignorespaces\the\DATE\vskip21pt}}%
}%
%
\tstmiss%
  {\THESAURUS}%
  {\infuser{^^JThesaurus codes are not given.}}%
  {\global\THESAURUS={missing; you have not inserted them}}%
  {}%
  {}%
%
\normalsize
%
\tstmiss%
  {\ABSTRACT}%
  {\missmsg{ABSTRACT}}%
  {\ABSTRACT={Not yet given.}}%
  {}%
  {\noindent{\bf Abstract. }\ignorespaces\the\ABSTRACT\vskip0.5true cm}%
%
\tstmiss%
  {\KEYWORDS}%
  {\missmsg{KEYWORDS}}%
  {\KEYWORDS={Not yet given.}}%
  {}%
  {\noindent{\bf Key words: }\ignorespaces\the\KEYWORDS
  \strich}%
%
\global\sterne=0
\global\catcode`\@=12
}\normalsize}%Ende von maketitle
% @ ist wieder ein ganz normales Zeichen und wird auch als solches
% gedruckt.
%-------------------------------------------------------------------
% This is twocolout.tex
% This file gives plain TeX the ability of single and double
% column output with floating insertions at the top which span
% both columns in double column format.
% The default format is double column format. Switching between
% single and double column format is provided but inserts
% an immediate page break and ejects all floating insertions.
% Double column floating insertions defined in text in a
% right column are held back until the beginning of the next page.
% -----------------------------------------------------------------
%
% Macros which the user should know about:
%
% \setuplr#1#2#3   : Should be called before any output
%                    #1 = O (one column) or T (two columns,default)
%                    #2 <dimen> = text width (both columns)
%                    #3 <dimen> = column width
%
% \newpage         : Fill a whole page and start a new one
% \newcolumn       : Start a new column
% \onecolumn       : Break the current page and switch to one column
% \twocolumns      : Break the current page and switch to two columns
%
% \bothtopinsert   : Beginning of a floating insertion over the
%                    full text width
% \endbothinsert   : End of such an insertion (analog to \endinsert)
% \specialpage     : Insert a special page following the current page
%
% All macros with a '@' in their names are for internal usage only.
%
% Modified macros for A&A:
%    \output \typeset \refereelayout
%    \titlea \titleb \titlec \titled
%    \begref \ref \endref \ack \app \figure
%    \begfig \begfigwid \begtab \begtabfullwid \begtabemptywid
% Original A&A macros using one of the modified macros:
%    \bye (\typeset)
% New macros for A&A:
%    \begfigpage \begtabempty \begtabfull \begtabpage
%    \puthere \putattop \putatbottom
% -----------------------------------------------------------------
%
\catcode`@=11    % use @ as a normal character
%
\newdimen\@txtwd  \@txtwd=\hsize
\newdimen\@txtht  \@txtht=\vsize
\newdimen\@colht  \@colht=\vsize
\newdimen\@colwd  \@colwd=-1pt
\newdimen\@colsavwd
%%%
%%% =========== Macros for initializing the whole thing ==========
%%%
\newcount\in@t \in@t=0
\def\initlr{\if N\lr \ifdim\@colwd<0pt \global\@colwd=\hsize \fi
   \else\global\let\lr=L\ifdim\@colwd<0pt \global\@colwd=\hsize
      \global\divide\@colwd\tw@ \global\advance\@colwd by -10pt
   \fi\fi\global\advance\in@t by 1}
\def\setuplr#1#2#3{\let\lr=O \ifx#1\lr\global\let\lr=N
      \else\global\let\lr=L\fi
   \@txtht=\vsize \@colht=\vsize \@txtwd=#2 \@colwd=#3
   \if N\lr \else\multiply\@colwd\tw@ \fi
   \ifdim\@colwd>\@txtwd\if N\lr
        \errmessage{The text width is less than the column width}%
      \else
        \errmessage{The text width is less the two times the column width}%
      \fi \global\@colwd=\@txtwd
      \if N\lr\divide\@colwd by 2\fi
   \else \global\@colwd=#3 \fi \initlr \@colsavwd=#3
   \global\@insmx=\@txtht
   \global\hsize=\@colwd}
%% ----------- switching between one and two column output ------
\def\twocolumns{\@fillpage\eject\global\let\lr=L \@makecolht
   \global\@colwd=\@colsavwd \global\hsize=\@colwd}
\def\onecolumn{\@fillpage\eject\global\let\lr=N \@makecolht
   \global\@colwd=\@txtwd \global\hsize=\@colwd}
\def\newpage{\@fillpage\eject}
\def\@fillpage{\vfill\supereject\if R\lr \null\vfill\eject\fi}
\def\newcolumn{\vfill\supereject}
%% ----------------------------------------------------------------
%%%
%%% =============== Macros used by the output routine ===============
%%%
\newbox\@leftcolumn
\newbox\@rightcolumn
\newbox\@outputbox
\newbox\@tempboxa
\newbox\@keepboxa
\newbox\@keepboxb
\newbox\@bothcolumns
\newbox\@savetopins
\newbox\@savetopright
\newcount\verybad \verybad=1010
%% -------- \@makecolumn puts the current column in a box ---------
\def\@makecolumn{\ifnum \in@t<1\initlr\fi
   \ifnum\outputpenalty=\the\verybad1  %%% i.e. 10101 if \verybad=1010
      \if L\lr\else\advance\pageno by1\fi
      \infuser{Warning: There is a 'widow' line
      at the top of page \the\pageno\if R\lr (left)\fi.
      This is unacceptable.} \if L\lr\else\advance\pageno by-1\fi \fi
   \ifnum\outputpenalty=\the\verybad2
      \infuser{Warning: There is a 'club' line
      at the bottom of page \the\pageno\if L\lr(left)\fi.
      This is unacceptable.} \fi
   \if L\lr \ifvoid\@savetopins\else\@colht=\@txtht\fi \fi
   \if R\lr \ifvoid\@bothcolumns \ifvoid\@savetopright
       \else\@colht=\@txtht\fi\fi\fi
   \global\setbox\@outputbox
   \vbox to\@colht{\boxmaxdepth\maxdepth
   % One-column top insertions are held back if there is already a
   % two-column floating insertion and the one-column top insertion
   % doesn't fit entirely in the column.
   \if L\lr \ifvoid\@savetopins\else\unvbox\@savetopins\fi \fi
   \if R\lr \ifvoid\@bothcolumns \ifvoid\@savetopright\else
       \unvbox\@savetopright\fi\fi\fi
   \ifvoid\topins\else\ifnum\count\topins>0
         \ifdim\ht\topins>\@colht
            \infuser{^^JError: Too many or too large single column
            box(es) on this page.}\fi
         \unvbox\topins
      \else
         \global\setbox\@savetopins=\vbox{\ifvoid\@savetopins\else
         \unvbox\@savetopins\penalty-500\fi \unvbox\topins} \fi\fi
   \dimen@=\dp\@cclv \unvbox\@cclv % open up \box255
   \ifvoid\bottomins\else\unvbox\bottomins\fi
   \ifvoid\footins\else % footnote info is present
     \vskip\skip\footins
     \footnoterule
     \unvbox\footins\fi
   \ifr@ggedbottom \kern-\dimen@ \vfil \fi}%
}
%% --------- \@outputpage puts the columns and the top insertions
%% --------- together and puts them out
\def\@outputpage{\@dooutput{\lr}}
\def\@colbox#1{\hbox to\@colwd{\box#1\hss}}
\def\@dooutput#1{\global\topskip=10pt
  \ifdim\ht\@bothcolumns>\@txtht
    \if #1N
       \unvbox\@outputbox
    \else
       \unvbox\@leftcolumn\unvbox\@outputbox
    \fi
    \global\setbox\@tempboxa\vbox{\hsize=\@txtwd\makeheadline
       \vsplit\@bothcolumns to\@txtht
       \makefootline\hsize=\@colwd}%
    \infuser{^^JError: Too many double column boxes on this page.}%
    \shipout\box\@tempboxa\advancepageno
    \unvbox255 \penalty\outputpenalty
  \else
    \global\setbox\@tempboxa\vbox{\hsize=\@txtwd\makeheadline
       \ifvoid\@bothcolumns\else\unvbox\@bothcolumns\fi
       \hsize=\@colwd
       \if #1N
          \hbox to\@txtwd{\@colbox{\@outputbox}\hfil}%
       \else
          \hbox to\@txtwd{\@colbox{\@leftcolumn}\hfil\@colbox{\@outputbox}}%
       \fi
       \hsize=\@txtwd\makefootline\hsize=\@colwd}%
    \shipout\box\@tempboxa\advancepageno
  \fi
  \ifnum \special@pages>0 \s@count=100 \page@command
      \xdef\page@command{}\global\special@pages=0 \fi
  }
%% -------- \balance@right@left balances the columns on the last
%% -------- page of text.
\def\balance@right@left{\dimen@=\ht\@leftcolumn
    \advance\dimen@ by\ht\@outputbox
    \advance\dimen@ by\ht\springer@macro
    \dimen2=\z@ \global\the@end=0
    % put both columns together and compensate \vfill at the end
    \ifdim\dimen@>70pt\setbox\z@=\vbox{\unvbox\@leftcolumn
          \unvbox\@outputbox}%
       \loop
          \dimen@=\ht\z@
          \advance\dimen@ by0.5\topskip
          \advance\dimen@ by\baselineskip
          \advance\dimen@ by\ht\springer@macro
          \advance\dimen@ by\dimen2
          \divide\dimen@ by2
          \splittopskip=\topskip
          % Now split it to two parts of about the same height
          {\vbadness=10000
             \global\setbox3=\copy\z@
             \global\setbox1=\vsplit3 to \dimen@}%
          \dimen1=\ht3 \advance\dimen1 by\ht\springer@macro
       \ifdim\dimen1>\ht1 \advance\dimen2 by\baselineskip\repeat
       \dimen@=\ht1
       % Restore the column boxes and adjust
       \global\setbox\@leftcolumn
          \hbox to\@colwd{\vbox to\@colht{\vbox to\dimen@{\unvbox1}\vfil}}%
       \global\setbox\@outputbox
          \hbox to\@colwd{\vbox to\@colht{\vbox to\dimen@{\unvbox3
             \vfill\box\springer@macro}\vfil}}%
    \else
       \setbox\@leftcolumn=\vbox{unvbox\@leftcolumn\bigskip
          \box\springer@macro}%
    \fi}
%
%%%
%%% ================== Insertion routines ======================
%%%
%%% This follows loosely the definition of \topins by Knuth but without
%%% the need to distinguish between 3 different kinds of insertions.
%%% See the TeXBook p.363.
%%% Insertions in right columns are first saved in a box (\rightins)
%%% and inserted to \bothins after this column has been shipped out.
%
\newinsert\bothins
\newbox\rightins
\skip\bothins=\z@skip
\count\bothins=1000
\dimen\bothins=\@txtht \advance\dimen\bothins by -\bigskipamount
\def\bothtopinsert{\par\begingroup\setbox\z@\vbox\bgroup
    \hsize=\@txtwd\parskip=0pt\par\noindent\bgroup}
\def\endbothinsert{\egroup\egroup
  \if R\lr
    \right@nsert
  \else    % L\lr or N\lr
    % If double column insertions don't fit into the current columm
    % keep them until the next page starts.
    \dimen@=\ht\z@ \advance\dimen@ by\dp\z@ \advance\dimen@ by\pagetotal
    \advance\dimen@ by \bigskipamount \advance\dimen@ by \topskip
    \advance\dimen@ by\ht\topins \advance\dimen@ by\dp\topins
    \advance\dimen@ by\ht\bottomins \advance\dimen@ by\dp\bottomins
    \advance\dimen@ by\ht\@savetopins \advance\dimen@ by\dp\@savetopins
    \ifdim\dimen@>\@colht\right@nsert\else\left@nsert\fi
  \fi  \endgroup}
\def\right@nsert{\global\setbox\rightins\vbox{\ifvoid\rightins
    \else\unvbox\rightins\fi\penalty100
    \splittopskip=\topskip
    \splitmaxdepth\maxdimen \floatingpenalty200
    \dimen@\ht\z@ \advance\dimen@\dp\z@
    \box\z@\nobreak\bigskip}}
\def\left@nsert{\insert\bothins{\penalty100
    \splittopskip=\topskip
    \splitmaxdepth\maxdimen \floatingpenalty200
    \box\z@\nobreak\bigskip}
    \@makecolht}
\newdimen\@insht    \@insht=\z@
\newdimen\@insmx    \@insmx=\vsize
%% ------ \@makecolht computes the available height of the current column.
\def\@makecolht{\global\@colht=\@txtht \@compinsht
    \global\advance\@colht by -\@insht \global\vsize=\@colht
    \global\dimen\topins=\@colht}
\def\@compinsht{\if R\lr
       \dimen@=\ht\@bothcolumns \advance\dimen@ by\dp\@bothcolumns
       \ifvoid\@bothcolumns \advance\dimen@ by\ht\@savetopright
          \advance\dimen@ by\dp\@savetopright \fi
    \else
       \dimen@=\ht\bothins \advance\dimen@ by\dp\bothins
       \advance\dimen@ by\ht\@savetopins \advance\dimen@ by\dp\@savetopins
    \fi
    \ifdim\dimen@>\@insmx
       \global\@insht=\dimen@
    \else\global\@insht=\dimen@
    \fi}
\newinsert\bottomins
\skip\bottomins=\z@skip
\count\bottomins=1000
%%%
%%% Special pages to be inserted
%%%
\xdef\page@command{}
\newcount\s@count
\newcount\special@pages \special@pages=0
\def\specialpage#1{\global\advance\special@pages by1
    \global\s@count=\special@pages
    \global\advance\s@count by 100
    \global\setbox\s@count
    \vbox to\@txtht{\hsize=\@txtwd\parskip=0pt
    \par\noindent\noexpand#1\vfil}%
    \def\protect{\noexpand\protect\noexpand}%
    \xdef\page@command{\page@command
         \protect\global\advance\s@count by1
         \protect\begingroup
         \protect\setbox\z@\vbox{\protect\makeheadline
                                    \protect\box\s@count
            \protect\makefootline}%
         \protect{\shipout\box\z@}%
         \protect\endgroup\protect\advancepageno}%
    \let\protect=\relax
   }
%%%
%%%
%%% This little macro adjusts the top of figure boxes with the
%%% the top of the column. Previously they were adjusted with the
%%% the baseline of the first row in a column.
\def\@startins{\vskip \topskip\hrule height\z@
   \nobreak\vskip -\topskip\vskip3.7pt}
%%%
%%%  ==============  The main output routine ===============
%%%
%%%           The output routine was adapted to A&A
%%%
\let\retry=N
\output={\@makecolht \global\topskip=10pt \let\retry=N%
   \ifnum\count\topins>0 \ifdim\ht\topins>\@colht
       \global\count\topins=0 \global\let\retry=Y%
       \unvbox\@cclv \penalty\outputpenalty \fi\fi
   \if N\retry
    \if N\lr     % this is for single column output
       \@makecolumn
       \ifnum\the@end>0
          \setbox\z@=\vbox{\unvcopy\@outputbox}%
          \dimen@=\ht\z@ \advance\dimen@ by\ht\springer@macro
          \ifdim\dimen@<\@colht
             \setbox\@outputbox=\vbox to\@colht{\box\z@
             \unskip\vskip12pt plus0pt minus12pt
             \box\springer@macro\vfil}%
          \else \box\springer@macro \fi
          \global\the@end=0
       \fi
       \ifvoid\bothins\else\global\setbox\@bothcolumns\box\bothins\fi
       \@outputpage
       \ifvoid\rightins\else
       %  Hold \rightins back if there is already a \@savetopins
       \ifvoid\@savetopins\insert\bothins{\unvbox\rightins}\fi
       \fi
    \else
       \if L\lr    % this is the left of two columns
          \@makecolumn
          \global\setbox\@leftcolumn\box\@outputbox \global\let\lr=R%
          \ifx Y\firstpage %\ifnum\pageno=1
             \infuser{^^J[left\the\pageno]}%
          \else
             \infuser{[left\the\pageno]}\fi
          \ifvoid\bothins\else\global\setbox\@bothcolumns\box\bothins\fi
          \global\dimen\bothins=\z@
          \global\count\bothins=0
          \ifx Y\firstpage %\ifnum\pageno=1
             \global\topskip=\fullhead\fi
       \else    % the right column
          \@makecolumn
          \ifnum\the@end>0\ifnum\pageno>1\balance@right@left\fi\fi
          \@outputpage \global\let\lr=L%
          \global\dimen\bothins=\maxdimen
          \global\count\bothins=1000
          \ifvoid\rightins\else
          %  Hold \rightins back if there is already a \@savetopins
             \ifvoid\@savetopins \insert\bothins{\unvbox\rightins}\fi
          \fi
       \fi
    \fi
    \global\let\last@insert=N \put@default
    \ifnum\outputpenalty>-\@MM\else\dosupereject\fi
    \ifvoid\@savetopins\else
      \ifdim\ht\@savetopins>\@txtht
        \global\setbox\@tempboxa=\box\@savetopins
        \global\setbox\@savetopins=\vsplit\@tempboxa to\@txtht
        \global\setbox\@savetopins=\vbox{\unvbox\@savetopins}%
        \global\setbox\@savetopright=\box\@tempboxa \fi
    \fi
    \@makecolht
    \global\count\topins=1000
   \fi
   }
%
%%% ----------  Start one- or two-column output  ---------
%
\if N\lr
   \setuplr{O}{\fullhsize}{\hsize}% O = one column
\else
   \setuplr{T}{\fullhsize}{\hsize}% T = two columns
\fi
% This is aafigure.tex
%
% The macros cover the case of single column format as well
% as double column format. In single column format all 'double
% column' insertions are reduced to single column insertions.
% While real double column insertions will always appear at
% the top of page, the placement of single column insertions
% can be influenced by the definition of \put@default.
% Possible positions are at the current position (only if
% \insert@here expands to Y, there is no top and no bottom insertion
% so far, and there is enough space), at the bottom of the column
% (only if \insert@at@the@bottom expands to Y and there is enough
% space in this column) and at the top of the column but below
% any double column insertion.
% The default placement of single column figures is usually at the top.
% If the figure almost fills the page if inserted at the bottom,
% it may go there.
%
\catcode`@=11
\def\put@default{\global\let\insert@here=Y
   \global\let\insert@at@the@bottom=N}%
% Allow figures to be inserted a the current position (if possible):
\def\puthere{\global\let\insert@here=Y%
    \global\let\insert@at@the@bottom=N}
% All figures are inserted at the top:
\def\putattop{\global\let\insert@here=N%
    \global\let\insert@at@the@bottom=N}
% Figures are inserted at the bottom (if possible):
\def\putatbottom{\global\let\insert@here=N%
    \global\let\insert@at@the@bottom=X}
%--------------------------------------------------------------------
\put@default
\let\last@insert=N        % Always reset to 'N' when a column is finished
\def\end@skip{\smallskip} % This space is added except after bottom insertions
\newdimen\min@top
\newdimen\min@here
\newdimen\min@bot
\min@top=10cm
\min@here=4cm   % do not insert figures after a few lines of text only
\min@bot=\topskip % figures may be at the bottom but there is a \@startins
\def\figfuzz{\vskip 0pt plus 6pt minus 3pt}  % more flexible spacing
%--------------------------------------------------------------------
\def\check@here@and@bottom#1{\relax
   %%% Several conditions have to be true if a figure or table can be
   %%% inserted at the current position or at the bottom of the page.
   %%% These conditions should preserve the
   %%% order of single column figures and put floating figures
   %%% always to the top of a column. However, exceptions are
   %%% possible with a \puthere\begfig{...}\endfig appearing at
   %%% the current position and a later \begfig{...}\endfig
   %%% appearing at the top of the same column.
   %
   \ifvoid\topins\else       \global\let\insert@here=N\fi
   \if B\last@insert         \global\let\insert@here=N\fi
   \if T\last@insert         \global\let\insert@here=N\fi
   \ifdim #1<\min@bot        \global\let\insert@here=N\fi
   \ifdim\pagetotal>\@colht  \global\let\insert@here=N\fi
   \ifdim\pagetotal<\min@here\global\let\insert@here=N\fi
   %
   \if X\insert@at@the@bottom\global\let\insert@at@the@bottom=Y
     \else\if T\last@insert  \global\let\insert@at@the@bottom=N\fi
          \if H\last@insert  \global\let\insert@at@the@bottom=N\fi
          \ifvoid\topins\else\global\let\insert@at@the@bottom=N\fi\fi
   \ifdim #1<\min@bot        \global\let\insert@at@the@bottom=N\fi
   \ifdim\pagetotal>\@colht  \global\let\insert@at@the@bottom=N\fi
   \ifdim\pagetotal<\min@top \global\let\insert@at@the@bottom=N\fi
   %
   \ifvoid\bottomins\else    \global\let\insert@at@the@bottom=Y\fi
   \if Y\insert@at@the@bottom\global\let\insert@here=N\fi }
%
\def\single@column@insert#1{\relax
   \setbox\@tempboxa=\vbox{#1}%
   \dimen@=\@colht \advance\dimen@ by -\pagetotal
   \advance\dimen@ by-\ht\@tempboxa \advance\dimen0 by-\dp\@tempboxa
   \advance\dimen@ by-\ht\topins \advance\dimen0 by-\dp\topins
   \check@here@and@bottom{\dimen@}%
   \if Y\insert@here
      \par  % The insertion forces a new paragraph in this case.
      \midinsert\figfuzz\relax     %%%%%%%%%\bigskip
      \box\@tempboxa\end@skip\figfuzz\endinsert
      \global\let\last@insert=H
   \else \if Y\insert@at@the@bottom
      \begingroup\insert\bottomins\bgroup\if B\last@insert\end@skip\fi
      \floatingpenalty=20000\figfuzz\bigskip\box\@tempboxa\egroup\endgroup
      \global\let\last@insert=B
   \else
      \topinsert\box\@tempboxa\end@skip\figfuzz\endinsert
      \global\let\last@insert=T
   \fi\fi\put@default\ignorespaces}
%
% ---------------- The insertion macros for the user -------------------
%
\def\begfig#1cm#2\endfig{\par\the\everypar
\single@column@insert{\@startins\rahmen{#1}#2}\ignorespaces}
\def\begfigwid#1cm#2\endfig{\par\the\everypar
   \if N\lr  % Here the only difference to \begfig is the larger \hsize
      {\hsize=\fullhsize \begfig#1cm#2\endfig}%
   \else
      \setbox0=\vbox{\hsize=\fullhsize\bigskip#2\smallskip}%
      \dimen0=\ht0\advance\dimen0 by\dp0
      \advance\dimen0 by#1cm
      \advance\dimen0by7\normalbaselineskip\relax
      \ifdim\dimen0>\@txtht
         \infuser{^^JFigure plus legend too high, will try to put it on a
                  separate page. }%
         \begfigpage#1cm#2\endfig
      \else
         \bothtopinsert\line{\vbox{\hsize=\fullhsize
         \@startins\rahmen{#1}#2\smallskip}\hss}\figfuzz\endbothinsert
      \fi
   \fi}
%
\def\begfigside#1cm#2cm#3\endfig{\par\the\everypar
   \if N\lr  % Here the only difference to \begfig is the larger \hsize
      {\hsize=\fullhsize \begfig#1cm#3\endfig}%
   \else
      \dimen0=#2true cm\relax
      \ifdim\dimen0<\hsize
         \infuser{^^JYour figure fits in a single column; why don't
                  ^^Jyou use \string\begfig\space instead of
                  \string\begfigside? }%
      \fi
      \dimen0=\fullhsize
      \advance\dimen0 by-#2true cm
      \advance\dimen0 by-1true cc\relax
      \bgroup
         \ifdim\dimen0<8true cc\relax
            \infuser{^^JNo sufficient room for the legend;
                     using \string\begfigwid. }%
            \begfigwid #1cm#3\endfig
         \else
            \ifdim\dimen0<10true cc\relax
               \infuser{^^JRoom for legend to narrow;
                        legend will be set raggedright. }%
               \rightskip=0pt plus 2cm\relax
            \fi
            \setbox0=\vbox{\def\figure##1##2{\vbox{\hsize=\dimen0\relax
                           \@startins\noindent\petit{\bf
                           Fig.\ts##1\unskip.\ }\ignorespaces##2\par}}%
                           #3\unskip}%
            \ifdim#1true cm<\ht0\relax
               \infuser{^^JText of legend higher than figure; using
                        \string\begfig. }%
               \begfigwid #1cm#3\endfig
            \else
               \def\figure##1##2{\vbox{\hsize=\dimen0\relax
                                       \@startins\noindent\petit{\bf
                                       Fig.\ts##1\unskip.\
                                       }\ignorespaces##2\par}}%
               \bothtopinsert\line{\vbox{\hsize=#2true cm\relax
               \@startins\rahmen{#1}}\hss#3\unskip}\figfuzz\endbothinsert
            \fi
         \fi
      \egroup
   \fi\ignorespaces}
%
\def\begfigpage#1cm#2\endfig{\par\the\everypar\specialpage{\@startins
   \vskip3.7pt\rahmen{#1}#2}\ignorespaces}%
\def\begtab#1cm#2\endtab{\par\the\everypar
\single@column@insert{#2\rahmen{#1}}\ignorespaces}
\let\begtabempty=\begtab
\def\begtabfull#1\endtab{\par\the\everypar
\single@column@insert{#1}\ignorespaces}
\def\begtabemptywid#1cm#2\endtab{\par\the\everypar
   \if N\lr
      {\hsize=\fullhsize \begtabempty#1cm#2\endtab}%
   \else
      \bothtopinsert\line{\vbox{\hsize=\fullhsize
      #2\rahmen{#1}}\hss}\medskip\endbothinsert
   \fi\ignorespaces}
\def\begtabfullwid#1\endtab{\par\the\everypar
   \if N\lr
      {\hsize=\fullhsize \begtabfull#1\endtab}%
   \else
      \bothtopinsert\line{\vbox{\hsize=\fullhsize
      \noindent#1}\hss}\medskip\endbothinsert
   \fi\ignorespaces}
\def\begtabpage#1\endtab{\par\the\everypar\specialpage{#1}\ignorespaces}
\catcode`@=12
% This is startup.aa
% It defines additional macros and settings that are special for
% the AA package or that have to be changed in the macros
% already loaded. A control sequence \firsttodo is defined that is
% called first after TeX starts up and is executed by \everyjob for
% a format file use of the package.
%
\catcode`@=11 % use @ as a normal character
%
\def\SpringerMacroPackageNameA{AA}
%
\edef\firsttodo{%
\infuser{^^JThis is \SpringerMacroPackageNameA, the plain TeX macro
package from Springer-Verlag,^^Jfor the Astronomy and Astrophysics
Main Journal
\ifx\Initexing\undefined\else format file \fi
\fonttype\space version 3.0^^J}%
\catcode`@=\active   % This is reset by the \maketitle macro
}
%
\everyjob={\firsttodo}% set the startup variable of TeX
\firsttodo % (do things that are first to do :-)
\catcode`@=12 % at signs are no longer letters
%%% rest removed from cp-aa.ini
%% This is dodump.aa
%% it clears the first page possibly filled with junk material
%% adjusts the page counter and calls INITEX's \dump
%\pageno=0
%\let\header=N%
%\leavevmode
%\vfil
%You just produced a \TeX{} format file for the \fonttype\space
%version of the {\tt\SpringerMacroPackageNameA} macro package from
%Springer-Verlag.
%\bigskip
%\vfil
%\eject
%\let\Initexing=\undefined
%\dump
%.
 

